Investigating the Effectiveness of ChatGPT in Mathematical Reasoning and Problem Solving: Evidence from the Vietnamese National High School Graduation Examination

This study offers a complete analysis of ChatGPT's mathematics abilities in responding to multiple-choice questions for the Vietnamese National High School Graduation Examination (VNHSGE) on a range of subjects and difficulty levels. The dataset included 250 questions divided into four levels: knowledge (K), comprehension (C), application (A), and high application (H), and it included ten themes that covered diverse mathematical concepts. The outcomes demonstrate that ChatGPT's performance varies depending on the difficulty level and subject. It performed best on questions at Level (K), with an accuracy rate of $83\%$; but, as the difficulty level rose, it scored poorly, with an accuracy rate of $10\%$. The study has also shown that ChatGPT significantly succeeds in providing responses to questions on subjects including exponential and logarithmic functions, geometric progression, and arithmetic progression. The study found that ChatGPT had difficulty correctly answering questions on topics including derivatives and applications, spatial geometry, and Oxyz spatial calculus. Additionally, this study contrasted ChatGPT outcomes with Vietnamese students in VNHSGE and in other math competitions. ChatGPT dominated in the SAT Math competition with a success rate of $70\%$, followed by VNHSGE mathematics ($58.8\%)$. However, its success rates were lower on other exams, such as AP Statistics, the GRE Quantitative, AMC 10, AMC 12, and AP Calculus BC. These results suggest that ChatGPT has the potential to be an effective teaching tool for mathematics, but more work is needed to enhance its handling of graphical data and address the challenges presented by questions that are getting more challenging.

==> level.tex <==
 75.00, 90.00, 81.82, 89.47, 85.71
 40.00, 72.22, 62.50, 62.50, 58.82
 25.00, 0.00, 28.57, 55.56, 20.00
 0.00, 0.00, 0.00, 16.67, 22.22


==> topic.tex <==
 50, 0, 50, 100,
 100, 100, 100, 100,
 50, 50, 100, 100,
 30, 50, 20, 46.1538461538462,
 75, 75, 75, 62.5,
 57.1428571428571, 71.4285714285714, 71.4285714285714, 42.8571428571429,
 83.3333333333333, 66.6666666666667, 66.6666666666667, 100,
 33.3333333333333, 66.6666666666667, 66.6666666666667, 66.6666666666667,
 50, 66.6666666666667, 66.6666666666667, 100,
 44.4444444444444, 62.5, 62.5, 75,

